Understanding the robustness difference between stochastic gradient descent and adaptive gradient methods

Stochastic gradient descent (SGD) and adaptive gradient methods, such as Adam and RMSProp, have been widely used in training deep neural networks. We empirically show that while the difference between the standard generalization performance of models trained using these methods is small, those trained using SGD exhibit far greater robustness under input perturbations. Notably, our investigation demonstrates the presence of irrelevant frequencies in natural datasets, where alterations do not affect models' generalization performance. However, models trained with adaptive methods show sensitivity to these changes, suggesting that their use of irrelevant frequencies can lead to solutions sensitive to perturbations. To better understand this difference, we study the learning dynamics of gradient descent (GD) and sign gradient descent (signGD) on a synthetic dataset that mirrors natural signals. With a three-dimensional input space, the models optimized with GD and signGD have standard risks close to zero but vary in their adversarial risks. Our result shows that linear models' robustness to $\ell_2$-norm bounded changes is inversely proportional to the model parameters' weight norm: a smaller weight norm implies better robustness. In the context of deep learning, our experiments show that SGD-trained neural networks have smaller Lipschitz constants, explaining the better robustness to input perturbations than those trained with adaptive gradient methods.

==> Commands.tex <==
%\newdimen\pHeight
%\pHeight=-32678sp
%\newdimen\pLower
%\pLower=-4096sp
%\newdimen\pLineWidth
%\pLineWidth=32678sp
%\newdimen\pKern
%\pKern=-276480sp
%\newdimen\pIR
%\pIR=-131072sp
%\newsavebox{\Cbox}
%\newsavebox{\vertCmplx}
%\newdimen\Cheight
%\newdimen\Cwidth
%\sbox{\Cbox}{\rm C}
%\Cheight=\ht\Cbox
%\Cwidth=\wd\Cbox
%\advance\Cheight by \pHeight
%\sbox{\vertCmplx}{\rule[\pLower]{\pLineWidth}{\Cheight}}
%\sbox{\Cbox}{\usebox{\Cbox}\kern\pKern\usebox{\vertCmplx}}
%\wd\Cbox=\Cwidth
%%\def\C{\usebox{\Cbox}}
%%\def\Re{{\rm I\kern\pIR R}}
%\def\Re{\mathbb{R}}
%\def\Nat{{\rm I\kern\pIR N}}
%\def\argmax{\mathop{\rm arg\,max}}
%\def\argmin{\mathop{\rm arg\,min}}
%\def\liminf{\mathop{\rm lim\,inf}}
%\def\log{\mathop{\rm log}}
%\def\Mean{{\bf Mean}}
%\def\Var{{\bf Var}}
%\def\Cov{{\bf Cov}}
%\def\exptE{{\bf E}}
%\def\diag{\mathop{\rm diag}}

%\def\A{{\mathcal{A}}}
%\def\C{{\mathcal{C}}}
%\def\D{{\mathcal{D}}}
%\def\E{{\mathcal{E}}}
%\def\F{{\mathcal{F}}}
%\def\G{{\mathcal{G}}}
%\def\H{{\mathcal{H}}}
%\def\I{{\mathcal{I}}}
%\def\J{{\mathcal{J}}}
%\def\L{{\mathcal{L}}}
%\def\M{{\mathcal{M}}}
%\def\N{{\mathcal{N}}}
%\def\O{{\mathcal{O}}}
%\def\P{{\mathcal{P}}}
%\def\Q{{\mathcal{Q}}}
%\def\R{{\mathcal{R}}}
%\def\S{{\mathcal{S}}}
%\def\T{{\mathcal{T}}}
%\def\U{{\mathcal{U}}}
%\def\V{{\mathcal{V}}}
%\def\W{{\mathcal{W}}}
%\def\X{{\mathcal{X}}}
%\def\Z{{\mathcal{Z}}}

%\def\vecalpha{{\boldsymbol{\alpha}}}
%\def\vectheta{{\boldsymbol{\theta}}}
%\def\vecpi{{\boldsymbol{\pi}}}
%\def\vecpsi{{\boldsymbol{\psi}}}
%\def\vecphi{{\boldsymbol{\phi}}}
%\def\vec0{{\boldsymbol{0}}}
%\def\vecf{{\boldsymbol{f}}}
%\def\veck{{\boldsymbol{k}}}
%\def\vecp{{\boldsymbol{p}}}
%\def\vecq{{\boldsymbol{q}}}
\def\vecu{{\boldsymbol{u}}}
%\def\vecv{{\boldsymbol{v}}}
\def\vecw{{\boldsymbol{w}}}
%\def\vecx{{\boldsymbol{x}}}
%\def\vecy{{\boldsymbol{y}}}
%\def\vecz{{\boldsymbol{z}}}

%\def\matSigma{{\boldsymbol{\Sigma}}}
%\def\matA{{\boldsymbol{A}}}
%\def\matC{{\boldsymbol{C}}}
%\def\matF{{\boldsymbol{F}}}
%\def\matG{{\boldsymbol{G}}}
%\def\matH{{\boldsymbol{H}}}
%\def\matI{{\boldsymbol{I}}}
%\def\matK{{\boldsymbol{K}}}
%\def\matU{{\boldsymbol{U}}}
%\def\matY{{\boldsymbol{Y}}}
%\def\matZ{{\boldsymbol{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% New Commands %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ol}[1]{{\tilde{#1}}}
\newcommand{\rn}{{\Re^n}}



%% ORIGINAL AND WORKING
% THEOREMS -------------------------------------------------------
\newtheorem{theorem}{Theorem}% \ifDissertation[chapter]\fi
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}%\ifDissertation[chapter]\fi
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{assumption}{Assumption}
% \theoremstyle{remark}
\newtheorem{remark}{Remark}% \ifDissertation[chapter]\fi


%\newtheorem{thm}{Theorem}
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{prop}[thm]{Proposition}
%%\newtheorem{definition}[thm]{Definition}
%%\theoremstyle{definition}
%%\newtheorem{defn}{Definition}
%%\theoremstyle{remark}
%%\newtheorem{rem}[thm]{Remark}
\newcounter{assumption}%[section]
\renewcommand{\theassumption}{A\arabic{assumption}}

\newenvironment{assumption}[1][]{\begin{trivlist}\item[] \refstepcounter{assumption}%
 \textbf{Assumption\ \theassumption\ #1} }{%\par\nobreak\noindent\sl\ignorespaces}{%
 \ifvmode\smallskip\fi\end{trivlist}}

%\newenvironment{proof}{{\bf Proof.}}{\hfill\rule{2mm}{2mm}\\}

\renewcommand{\AA}{{\mathcal{A}}}
\newcommand{\C}{{\mathcal C}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\MS}{{\mathcal{S}}}
\newcommand{\TT}{{\mathcal{T}}}
\newcommand{\XX}{{\mathcal{X}}}
\newcommand{\YY}{{\mathcal{Y}}}
\newcommand{\ZZ}{{\mathcal{Z}}}
\newcommand{\XA}{\XX\times\AA}
\newcommand{\BX}{B(\XX)}
\newcommand{\BXA}{B(\XA)}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\Lip}{{\mathrm{Lip}}}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\vecalpha}{\boldsymbol{\alpha}}
\newcommand{\vecbeta}{\boldsymbol{\beta}}
\newcommand{\vectalpha}{\tilde{\vecalpha}}
\newcommand{\vecr}{\boldsymbol{r}}
\newcommand{\matA}{\boldsymbol{A}}
\newcommand{\matB}{\boldsymbol{B}}
\newcommand{\matC}{\boldsymbol{C}}
\newcommand{\matD}{\boldsymbol{D}}
\newcommand{\matE}{\boldsymbol{E}}
\newcommand{\matF}{\boldsymbol{F}}
\newcommand{\matG}{\boldsymbol{G}}
\newcommand{\matK}{\boldsymbol{K}}
\newcommand{\matI}{\boldsymbol{I}}
\newcommand{\kernelk}{\mathrm{k}}

% \newcommand{\kfun}{\mathrm{k}}
\newcommand{\kfun}{\textsc{k}}


\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\een}{\end{eqnarray*}}

\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
%\newcommand{\smallnorm}[1]{||#1||} % Previous version
\newcommand{\smallnorm}[1]{\Vert#1\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
%\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\set}[2]{\left\{\,#1\,:\,#2\,\right\}}
\newcommand{\Real}{\mathbb R}
\newcommand{\real}{\mathbb R}
%\newcommand{\Prob}[1]{{\mathbb P}\left(#1\right)} % It used to be ( )
\newcommand{\Prob}[1]{{\mathbb P}\left\{#1\right\}}
\newcommand{\EE}[1]{{\mathbb E}\left[#1\right]}
\newcommand{\EEn}[1]{\mathbb{E}_n\left[#1\right]}
\newcommand{\Var}[1]{{\mathrm{Var}}\left[#1\right]}
\renewcommand{\natural}{\mathbb{N}}
%\newcommand{\one}{\mathbb I}
\newcommand{\one}[1]{{\mathbb I}_{\{#1\}}}
\newcommand{\unit}{\mathbf 1}
\newcommand{\zero}{\mathbf 0}
\newcommand{\eps}{\varepsilon}
\newcommand{\ep}{\varepsilon}
\newcommand{\de}{\delta}
\newcommand{\To}{\longrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\yy}{{\bf y}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\F}{{\mathcal{F}}}
\newcommand{\FF}{{\mathcal{F}}}
\newcommand{\GG}{{\mathcal{G}}}
\newcommand{\GGA}{\GG^\actionnum}
\newcommand{\G}{{\mathcal{G}}}
\newcommand{\LL}{{\mathcal{L}}}
\newcommand{\NN}{{\mathcal{N}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\hs}{\hat{s}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hpi}{{\hat{\pi}}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\tQ}{\tilde{Q}}
\newcommand{\tih}{\tilde{h}}
\newcommand{\argmin}{\mathop{\textrm{argmin}}}
\newcommand{\argmax}{\mathop{\textrm{argmax}}}
\newcommand{\diag}{\mathop{\textrm{diag}}}
\newcommand{\hu}{\hat{u}}
\newcommand{\munorm}[1]{\norm{#1}_{\mu}}
\newcommand{\hmunorm}[1]{\norm{#1}_{\hat{\mu}}}
\newcommand{\Vmax}{V_{\textrm{max}}}
\newcommand{\Qmax}{Q_{\textrm{max}}} 
\newcommand{\Rmax}{R_{\textrm{max}}}
\newcommand{\hRmax}{\hat{R}_{\textrm{max}}}
\newcommand{\tRmax}{\tilde{R}_{\textrm{max}}}
\newcommand{\hLN}{\hat{L}_N}
\newcommand{\hpmunorm}[1]{\norm{#1}_{p,\hat{\mu}}}
\newcommand{\smallhpmunorm}[1]{\smallnorm{#1}_{p,\hat{\mu}}}


\newcommand{\pmunorm}[1]{\norm{#1}_{p,\mu}}
\newcommand{\pnunorm}[1]{\norm{#1}_{p,\nu}}
\newcommand{\smallpmunorm}[1]{\smallnorm{#1}_{p,\mu}}
\newcommand{\prhonorm}[1]{\norm{#1}_{p,\rho}}
\newcommand{\rhonorm}[1]{\norm{#1}_{\rho}}
\newcommand{\nunorm}[1]{\norm{#1}_{\nu}}
\newcommand{\nunormsmall}[1]{\|#1\|_{\nu}}
\newcommand{\supnorm}[1]{\norm{#1}_\infty}
% \newcommand{\R}{{\mathbb{R}}} 
%\newcommand{\eqdef}{\stackrel{\mbox{\text{\tiny def}}}{=}}
\newcommand{\eqdef}{\triangleq}


\newcommand{\xx}{{x_1,\ldots,x_N}}
\newcommand{\NdeClogs}{\Lambda} %LEGYEN INDEXE ??
\newcommand{\logplus}[1]{\log^+{#1}}
\newcommand{\VFx}{V_{\FF^{\times}}}
\newcommand{\FFx}{\FF^{\vee}}
\newcommand{\inlinemin}{\wedge}
\newcommand{\inlinemax}{\vee}
\newcommand{\obeta}{\overline{\beta}}
%\newcommand{\dimX}{{d_{\XX}}} ?
\newcommand{\VFp}{{V_{\FF^+}}}
\newcommand{\tEone}{\tilde{E}_1}
\newcommand{\ip}[2]{\left \langle\,#1\,,\,#2\, \right \rangle}
\newcommand{\behav}{{\pi_b}}
\newcommand{\behavbound}{{\pi_{b_0}}}
\newcommand{\actionnum}{{|\AA|}}
\newcommand{\actionnumsq}{M_2}
\newcommand{\FFA}{\FF^\actionnum}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\Pen}{J} %{\mathrm{Pen}}}



%\newcommand{\hstar}{h^*} % Previously used!
\newcommand{\hstar}{{\hat{h}_n}} % New
\newcommand{\htilde}{\tilde{h}}
\newcommand{\empnormsq}[1]{\left\Vert#1\right\Vert^2_n}
\newcommand{\empnorm}[1]{\left\Vert#1\right\Vert_n}
\newcommand{\empnormDnsq}[1]{\left\Vert#1\right\Vert^2_{\Dn}}
\newcommand{\empnormDn}[1]{\left\Vert#1\right\Vert_{\Dn}}

\newcommand{\smallempnorm}[1]{\Vert#1\Vert_n}
\newcommand{\smallempnormsq}[1]{\Vert#1\Vert^2_n}


\newcommand{\Qpi}{Q^\pi}
\newcommand{\Tpi}{T^\pi}
\newcommand{\Tpihat}{\hat{T}^\pi}
\newcommand{\Topt}{{T^*}}
\newcommand{\Topthat}{{\hat{T}^*}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\SobolevSpace}{\mathbb{W}^k(\Real^d)}
\newcommand{\SobolevSpaceM}{[\mathbb{W}^k(\Real^d)]^M}
\newcommand{\Jk}{J^2_k}
\newcommand{\J}{J^2}

\newcommand{\lambdaQ}{\lambda_{Q,n}}
\newcommand{\lambdaf}{\lambda_{f,n}}
\newcommand{\lambdah}{\lambda_{h,n}}


\newcommand{\HHA}{\HH^\actionnum}
\newcommand{\tZ}{\tilde{Z}}
\newcommand{\talpha}{\tilde{\alpha}}
\newcommand{\tmatK}{\tilde{\matK}}
\newcommand{\Op}{O_P} 

% \newcommand{\todo}[1]{{\textbf{[#1]}}}
%\usepackage{todonotes}


% New for My Thesis Proposal
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\rhatn}{\hat{r}_n}
\newcommand{\Dn}{\mathcal{D}_n}
\newcommand{\Dnk}{\mathcal{D}_{n,k}}

\newcommand{\FpC}{\mathcal{F}^{(p,C)}}
\newcommand{\DpC}{\mathcal{D}^{(p,C)}}


\newcommand{\Manifold}{\mathcal{M}}

\newcommand{\Id}{\mathbf{I}}

\newcommand{\R}{\mathcal{R}}

\newcommand{\EEX}[2]{{\mathbb E}_{#1}\left[#2\right]}


\newcommand{\Qopt}{Q^*}
\newcommand{\Vpi}{V^\pi}
\newcommand{\Vopt}{V^*}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\Vpihat}{\hat{V}^\pi}




% These have been defined somewhere else by someone else!
\newcommand{\bep}{\overline{\varepsilon}}
\newcommand{\pis}{{\pi^*}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\ModelsNo}{P}
\newcommand{\pistarhat}{\hat{\pi}^*}
\newcommand{\Ttilde}{\tilde{T}}

\newcommand{\TtildeQ}{\tilde{Q}}

\newcommand{\EmpLossRL}{\hat{L}^{\text{RL}}}
\newcommand{\EmpLoss}{\hat{L}}
\newcommand{\EmpRiskRL}{\mathcal{R}^\text{RL}}
\newcommand{\EmpRisk}{\mathcal{R}}

\newcommand{\LossRL}{L^{\text{RL}}}
%
\newcommand{\EmpBiasedLoss}{\hat{\tilde{L}}}
\newcommand{\BiasedLoss}{\tilde{L}}



\newcommand{\Ckn}{C_k(n)}
\newcommand{\Ck}{C_k}

\newcommand{\BadSetalpha}{\mathcal{A}_\alpha}


%\newcommand{\Ckdef}{\frac{20K\tau\,\ln k}{3\,a (1-a)\,n}}
\newcommand{\Ckdef}{\frac{4K \tau \ln k}{a (1-a)^2 \,n}}

%
%\newif \ifold
%\oldfalse
%%\oldtrue


\newcommand{\jhat}{\hat{j}}
\newcommand{\jhatk}{\hat{j}_k}
\newcommand{\jstar}{j_k^*}

\newcommand{\Qtilde}{\TtildeQ}
\newcommand{\khat}{{\hat{k}}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\Rem}{\Delta_1}
\newcommand{\MOSTE}[1]{
 \frac{\ln(\frac{2 c_5}{#1})}{c_2} + \frac{(1-a^2) \ln(\frac{2 c_6}{#1})}{c_4}}
\newcommand{\GoodEvent}{\mathcal{E}}

% Some names
%\newcommand{\RLMSProc}{\ensuremath{\mbox{\sc BEMoS}}}
\newcommand{\RLMSProc}{\ensuremath{\mbox{\textsc{BErMin}}}}
\newcommand{\RegProc}{\ensuremath{\mbox{\textsc{Regress}}}}


\newcommand{\bbarnk}{\bar{b}_{k,n}(\delta)}
\newcommand{\bbarnkdelta}{\bar{b}_{k,n}\left(\tfrac{2}{\pi^2}\tfrac{\delta}{k^2}\right)}
\newcommand{\OO}{{\mathcal{O}}}

\newcommand{\Alg}{{\textsf{A}}}
%\newcommand{\cA}{{\mathcal{A}}}
%\newcommand{\cA}{{\textsf{A}}}
\newcommand{\cset}[2]{\left\{\,#1\,:\,#2\,\right\}}


% For Excess Error Estimation section
\newcommand{\taumax}{{\tau_{\text{max}}}}
\newcommand{\bkdelta}[1]{{b(n,#1,\FF_k,\tau)}}
\newcommand{\gap}{\mathbf{g}}


\newcommand{\RLMSProcConst}{2} % was 3


\newcommand{\approxerror}{\mathfrak{A}}
\newcommand{\esterror}{\mathfrak{B}}
\newcommand{\bkdeltav}[1]{\esterror_k(n,#1,\tau)}
\newcommand{\Dmn}{{\mathcal{D}}_{(m,n)}}
\newcommand{\Dm}{{\mathcal{D}}_m}
\newcommand{\Dmk}{{\mathcal{D}}_{m,k}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% MDP-related definitions

\newcommand{\Set}{S}
\newcommand{\States}{\mathcal{X}}
\newcommand{\Actions}{\mathcal{A}}
\newcommand{\TranKernel}{\mathcal{P}}
\newcommand{\PKernel}{\mathcal{P}}
\newcommand{\RKernel}{\mathcal{R}}
\newcommand{\state}{x}
%\newcommand{\State}{X}
\newcommand{\action}{a}
\newcommand{\Action}{A}
\newcommand{\reward}{r}
\newcommand{\Reward}{R}
%\newcommand{\Return}{\mathcal{R}}
\newcommand{\MDP}{\mathcal{M}}
%\newcommand{\nextstate}{y}
%\newcommand{\Nextstate}{Y}
\newcommand{\nextstate}{x'}
\newcommand{\Nextstate}{X'}
\newcommand{\rewardfun}{r}
\newcommand{\TransPOp}{P}
\newcommand{\rmax}{r_{\max}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% For API
%\newcommand{\CrnuPI}{c_{1,\rho,\nu}}
%\newcommand{\CrnuPITwo}{c_{2,\rho,\nu}}
%\newcommand{\CrstarnuPI}{c'_{1,\rho^*,\nu}}

\newcommand{\CrnuPI}{c_{\text{PI}_1,\rho,\nu}}
\newcommand{\CrnuPITwo}{c_{\text{PI}_2,\rho,\nu}}
\newcommand{\CrstarnuPI}{c'_{\text{PI}_1,\rho^*,\nu}}
\newcommand{\CrnuPIPStar}{c_{\text{PI}_3,\rho,\nu}}

% For AVI
%\newcommand{\CrnuVI}{c_{4,\rho,\nu}} % Used to be this.
\newcommand{\CrnuVI}{c_{\text{VI}_1,\rho,\nu}}
\newcommand{\CrnuVITwo}{c_{\text{VI}_2,\rho,\nu}}

%\newcommand{\Popt}{P^*}
\newcommand{\Popt}{{P^{\pi^*}}}

\newcommand{\Tpik}{T^{\pi_k}}

\newcommand{\Tpiopt}{{T^{\pi^*}}}
\newcommand{\PpiK}{ {P^{\pi_K}} }


\newcommand{\twopnunorm}[1]{\norm{#1}_{2p,\nu}}

\newcommand{\epsBR}{\eps^\text{BR}}
\newcommand{\epsAE}{\eps^{\text{AE}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Zbar}{{\underline{Z}}}
\newcommand{\Zbarn}{{\underline{Z}_n}}

\newcommand{\zbar}{{\underline{z}}}
\newcommand{\zbarn}{{\underline{z}_n}}


\newcommand{\fbar}{\bar{f}}
\newcommand{\empnormmu}[1]{\left\Vert#1\right\Vert_{\mu_n}}
\newcommand{\empnormHmu}[1]{\left\Vert#1\right\Vert_{\Zbar(H_{1:\mun})}}
\newcommand{\empnormTmu}[1]{\left\Vert#1\right\Vert_{\Zbar(T_{1:\mun})}}




\newcommand{\empnormmusq}[1]{\left\Vert#1\right\Vert^2_{\mu_n}}
\newcommand{\empnormHmusq}[1]{\left\Vert#1\right\Vert^2_{\Zbar(H_{1:\mun})}}
\newcommand{\empnormTmusq}[1]{\left\Vert#1\right\Vert^2_{\Zbar(T_{1:\mun})}}

\newcommand{\empnormznsq}[1]{\left\Vert#1\right\Vert^2_{z_{1:n}}}
\newcommand{\empnormzn}[1]{\left\Vert#1\right\Vert_{z_{1:n}}}

\newcommand{\empnormzHmu}[1]{\left\Vert#1\right\Vert_{\zbar(H_{1:\mun})}}
\newcommand{\empnormzHmusq}[1]{\left\Vert#1\right\Vert^2_{\zbar(H_{1:\mun})}}

\newcommand{\FFbar}{{\bar{\FF}}}

\newcommand{\mun}{{\mu_n}}
\newcommand{\an}{{a_n}}
%\newcommand{\Residual}{{R_{\text{es}}}}
\newcommand{\Residual}{\mathcal{R}}

\newcommand{\blocka}{a_{n,l}}
\newcommand{\blockmu}{\mu_{n,l}}
%\newcommand{\BlockResidual}{{R_{\text{es},l}}}
\newcommand{\BlockResidual}{\mathcal{R}_l}



\newcommand{\mhatn}{\hat{m}_n}
\newcommand{\mtilden}{\tilde{m}_n}
\newcommand{\lambdan}{{\lambda_n}}
\newcommand{\Pensq}{\Pen^2}


% These are only used in the proof

\newcommand{\Anotation}{ {\log(\frac{1}{\beta} \max \{\log n, \ln(\frac{1}{\delta}) \}) }}
\newcommand{\Anotationwolog}{ {\frac{1}{\beta} \max \{\log n, \ln(\frac{1}{\delta}) \} }}
\newcommand{\Bnotation}{ {\log\Pensq(m) + \log n}}

\newcommand{\Tone}{T_{1,n}}
\newcommand{\Ttwo}{T_{2,n}}

\newcommand{\Ione}{I_{1,n}}
\newcommand{\Itwo}{I_{2,n}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\newcommand{\Dm}[1]{\mathcal{D}_{m_#1}}
%\newcommand{\Dm}[1]{\mathcal{D}^{(#1)}}
\newcommand{\Dataset}[1]{\mathcal{D}^{(#1)}}
\newcommand{\empnormsqm}[2]{\left\Vert#1\right\Vert^2_{m_{#2}}}
\newcommand{\empnormm}[2]{\left\Vert#1\right\Vert_{m_{#2}}}

\newcommand{\empnormsqD}[2]{\left\Vert#1\right\Vert^2_{\Dataset{#2}}}

\newcommand{\ProjFF}[1]{ {\Pi}_{\FF_{#1}} }
\newcommand{\ProjFFA}[1]{ {\Pi}_{\FFA_{#1}} }

\newcommand{\ProjFFnuX}[1]{ {\Pi}_{\nu_{\XX},\FF_{#1}} }
\newcommand{\ProjFFAnu}[1]{ {\Pi}_{\nu,\FFA_{#1}} }


% Used in RFQI-ApproxErrorPropagation
\newcommand{\FFAbar}{{\bar{\FF}^\actionnum}}

\newcommand{\diampnu}{\text{diam}_{p,\nu}}
\newcommand{\diam}{\text{diam}}


\newcommand{\CApproxErr}{c_{\text{AE},\nu}} % Remove this! 
\newcommand{\CApproxErrTwo}{C_{\text{AE}}(\nu;P)}
\newcommand{\CApproxErrTwoSquared}{C^2_{\text{AE}}(\nu;P)}

% Used in RFQI-SmoothnessPropagation
\newcommand{\JZTrans}{\mathcal{J}}


% Some other notations
\newcommand{\Argmin}{\mathop{\textrm{Argmin}}}
\newcommand{\Argmax}{\mathop{\textrm{Argmax}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\vecphi}{\boldsymbol{\phi}}
\newcommand{\matPhi}{\boldsymbol{\Phi}}
\newcommand{\matPsi}{\boldsymbol{\Psi}}

%%% Used in the proof
\newcommand{\Gsigma}{ {G_{\sigma_1,\sigma_2} }}
\newcommand{\GsigmaBRM}{ {G^\text{BRM}_{\sigma_1,\sigma_2} }}
\newcommand{\GsigmaLSTD}{ {G^\text{LSTD}_{\sigma_1,\sigma_2} }}

\newcommand{\gQh}{g_{Q,h}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\newcommand{\gapQ}{{\mathbf{g}_Q}}
\newcommand{\gapQ}{{\mathbf{g}_{Q^*}}}
\newcommand{\ProbWRT}[2]{{\mathbb P}_{#1}\left(#2\right)}
\newcommand{\One}[1]{{\mathbb I}{\{#1\}}}
\newcommand{\pihat}{{\hat{\pi}}}
\newcommand{\piopt}{{\pi^*}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\QpiPrime}{{Q^{\pi'}}}
\newcommand{\QpiPrimehat}{{\hat{Q}^{\pi'}}}
\newcommand{\gapQPrime}{{\mathbf{g}_\QpiPrime}}
\newcommand{\gapQPrimehat}{{\mathbf{g}_\QpiPrimehat}}

\newcommand{\pioptInPi}{ {\pi^*_\Pi} }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\newcommand{\QpiPrime}{{Q^{\pi'}}}
%\newcommand{\QpiPrimehat}{{\hat{Q}^{\pi'}}}
%\newcommand{\gapQPrime}{{\mathbf{g}_\QpiPrime}}
%\newcommand{\gapQPrimehat}{{\mathbf{g}_\QpiPrimehat}}
%
%\newcommand{\pioptInPi}{ {\pi^*_\Pi} }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\Dictionary}{{\mathcal B}}
\newcommand{\Dictionaryhat}{\hat{{\mathcal B}}}

\newcommand{\mhat}{\hat{m}}

%\newcommand{\COneStepAveraged}{C_\nu}
\newcommand{\COneStepAveraged}{C_{\nu \to \infty}}

\newcommand{\Penaltyn}{\mathrm{Pen}_n}
\newcommand{\LOneNonlinear}[2]{\mathcal{L}_1(#1;#2)}
\newcommand{\LOneNonlinearr}[2]{\mathcal{L}_{1,\alpha}(#1;#2)}

\newcommand{\Tthree}{T_{3,n}}
\newcommand{\Tfour}{T_{4,n}}


\newcommand{\actorparam}{{\theta^\mu}}
\newcommand{\criticparam}{{\theta^Q}}
\newcommand{\CKernel}{\mathcal{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ToptP}[1]{{T^*_{#1}}}
\newcommand{\TpiP}[1]{{T^{\pi}_{#1}}}

\newcommand{\KL}{\textsf{KL} }
\newcommand{\PKernelhat}{\hat{\PKernel} }
\newcommand{\PKernelTrue}{\PKernel^*}
\newcommand{\PKernelBestApprox}{{\tilde{\PKernel}}}
\newcommand{\Phat}{\hat{P} }

\newcommand{\PKernelpihat}{\hat{\PKernel}^{\pi} }
\newcommand{\PKernelpiTrue}{{\PKernel^*}^{\pi}}

%\newcommand{\AlgPlan}{{\textsf{A}_{\textsf{Plan}}}}
\newcommand{\AlgPlan}{{{\textsf{Planner}}}}
\newcommand{\Qopthat}{\hat{Q}^*}
\newcommand{\Vopthat}{\hat{V}^*}



\newcommand{\dx}{\mathrm{d}x}
\newcommand{\dy}{\mathrm{d}y}
\newcommand{\dz}{\mathrm{d}z}
\newcommand{\dmu}{\mathrm{d}\mu}
\newcommand{\dnu}{\mathrm{d}\nu}
\newcommand{\drho}{\mathrm{d}\rho}

\newcommand{\Ours}{{\text{SOAR}}}
\newcommand{\AdvOne}{{\text{Adv1}}}
\newcommand{\AdvSeven}{{\text{Adv7}}}
\newcommand{\Standard}{{\text{Standard}}}
\newcommand{\AdvOneScratch}{{\text{Adv1-scratch}}}
\newcommand{\AdvOnePretrain}{{\text{Adv1-pretrain}}}
\newcommand{\FGSM}{\text{FGSM}}
\newcommand{\PGD}{{\text{PGD}}}
\newcommand{\PGDOne}{{\text{PGD$1$}}}
\newcommand{\PGDTwenty}{{\text{PGD$20$}}}
\newcommand{\PGDSeven}{{\text{PGD$7$}}}
\newcommand{\LTwoPGD}{{\text{$\ell_{2}$-PGD}}}
% \newcommand{\LinfPGD}{ {\text{$\ell_{\infty}$-PGD}} }
\newcommand{\LinfPGD}{{\text{$\ell_{\infty}$-PGD}}}
\newcommand{\LTwo}{{\text{$\ell_{2}$}}}
\newcommand{\Linf}{{\text{$\ell_{\infty}$}}}
\newcommand{\Lp}{{\text{$\ell_{p}$}}}

\newcommand{\ResNet}{{-R}}
\newcommand{\WideResNet}{{-W}}


% \newcommand{\Ours}{ {\emph{SOAR}} }
% \newcommand{\AdvOne}{ {\emph{Adv1}} }
% \newcommand{\AdvSeven}{ {\emph{Adv7}} }
% \newcommand{\Standard}{ {\emph{Standard}} }
% \newcommand{\AdvOneScratch}{ {\emph{Adv1-scratch}} }
% \newcommand{\AdvOnePretrain}{ {\emph{Adv1-pretrain}} }
% \newcommand{\FGSM}{ {\emph{FGSM}} }
% \newcommand{\PGD}{ {\emph{PGD}} }
% \newcommand{\PGDOne}{ {\emph{PGD$1$}} }
% \newcommand{\PGDTwenty}{ {\emph{PGD$20$}} }
% \newcommand{\PGDSeven}{ {\emph{PGD$7$}} }
% \newcommand{\LTwoPGD}{ {\emph{$\ell_{2}$-PGD}} }
% \newcommand{\LinfPGD}{ {\emph{$\ell_{\infty}$-PGD}} }



\def\WW{{\mathcal{W}}}

\def\boxit#1#2{%
    \smash{\color{red}\fboxrule=1pt\relax\fboxsep=2pt\relax%
    \llap{\rlap{\fbox{\phantom{\rule{#1}{#2}}}}~}}\ignorespaces
}


\newcommand{\tx}{\tilde{x}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\te}{\tilde{e}}
